Harvard Glaucoma Detection and Progression: A Multimodal Multitask Dataset and Generalization-Reinforced Semi-Supervised Learning

Glaucoma is the number one cause of irreversible blindness globally. A major challenge for accurate glaucoma detection and progression forecasting is the bottleneck of limited labeled patients with the state-of-the-art (SOTA) 3D retinal imaging data of optical coherence tomography (OCT). To address the data scarcity issue, this paper proposes two solutions. First, we develop a novel generalization-reinforced semi-supervised learning (SSL) model called pseudo supervisor to optimally utilize unlabeled data. Compared with SOTA models, the proposed pseudo supervisor optimizes the policy of predicting pseudo labels with unlabeled samples to improve empirical generalization. Our pseudo supervisor model is evaluated with two clinical tasks consisting of glaucoma detection and progression forecasting. The progression forecasting task is evaluated both unimodally and multimodally. Our pseudo supervisor model demonstrates superior performance than SOTA SSL comparison models. Moreover, our model also achieves the best results on the publicly available LAG fundus dataset. Second, we introduce the Harvard Glaucoma Detection and Progression (Harvard-GDP) Dataset, a multimodal multitask dataset that includes data from 1,000 patients with OCT imaging data, as well as labels for glaucoma detection and progression. This is the largest glaucoma detection dataset with 3D OCT imaging data and the first glaucoma progression forecasting dataset that is publicly available. Detailed sex and racial analysis are provided, which can be used by interested researchers for fairness learning studies. Our released dataset is benchmarked with several SOTA supervised CNN and transformer deep learning models. The dataset and code are made publicly available via \url{https://ophai.hms.harvard.edu/datasets/harvard-gdp1000}.

==> sec/dataset.tex <==
\section{Dataset Analysis}

Two of major reasons why the medical data are high-variance: 
1) anatomy differences, from person to person
2) the progression process will make structural data at a point ambigous, i.e, they can be similar to both progression and non-progression samples.

==> sec/sec_broader_impact.tex <==


% \section*{Broader Impact}

% This research studies a new learning paradigm that leverages information in the training steps to improve the descent. Being model agnostic and general, the method will advance and enrich the fundamental research in machine learning. The more efficient and effective search of local minimum that facilitates the learning process will also bring significant impacts in developing automatic systems in a wide range of domains including education, healthcare, e-commerce, and many more. As other machine learning methods, systems derived with the method may fall short in performance or interpretability. While the proposed method shows improved performance, depending on specific domains or applications with varied requirements, precautions may need to be taken accordingly before using the automatic systems. This work, targeting an generic learning framework rather than a specific task or application, does not foresee particular ethical concerns in any specific areas or societal consequences. For a broader impact, we release the software of our research to the public. The source code is %attached in the Supplementary Materials. It is also 
% available at \url{https://rb.gy/qx1kuu}.


%This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. 
%This work is generic and its ultimate motivation is to benefit a broad variety of areas, \eg healthcare, education, economy, and etc, for human's material well-being.
%On the other hand, as the proposed method facilitates the learning process for applications, rather than implementing specific applications, 
%we believe that even the proposed work is modified for malevolent purposes, the resulting method would not harm humans and other morally relevant beings. 
%Because the proposed method is an essential tool for applications and is neutral to applications, and any modified version of this work cannot determine or re-shape the downstream applications. 
% In summary, this work has no direct link to malevolent applications.
%Therefore, this work does not present any foreseeable societal consequence.

% reference: The Ethics of Artificial Intelligence (published paper) and my imagination

%---------------previous version starts from here------------------
% This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. Our primary motivation is to provide a new perspective on the gradient descent that looks for a new direction to descend. The proposed method is generic and can apply to train models for other problems. As a result, the boosted model could used for both malicious and benevolent purposes. Nevertheless, the algorithmic impact of the proposed method has no direct link to malevolent applications and does not break the code of ethics.

% reference: https://hub.packtpub.com/machine-learning-ethics-what-you-need-to-know-and-what-you-can-do/

%---------------requirement starts from here------------------
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}
